Unified Multi-Task Learning & Model Fusion for Efficient Language Model Guardrailing

The trend towards large language models (LLMs) for guardrailing against undesired behaviors is increasing and has shown promise for censoring user inputs. However, increased latency, memory consumption, hosting expenses and non-structured outputs can make their use prohibitive. In this work, we show that task-specific data generation can lead to fine-tuned classifiers that significantly outperform current state of the art (SoTA) while being orders of magnitude smaller. Secondly, we show that using a single model, \texttt{MultiTaskGuard}, that is pretrained on a large synthetically generated dataset with unique task instructions further improves generalization. Thirdly, our most performant models, \texttt{UniGuard}, are found using our proposed search-based model merging approach that finds an optimal set of parameters to combine single-policy models and multi-policy guardrail models. % On 7 public datasets and 4 guardrail benchmarks we created, our efficient guardrail classifiers improve over the best performing SoTA publicly available LLMs and 3$^{\text{rd}}$ party guardrail APIs in detecting unsafe and safe behaviors by an average F1 score improvement of \textbf{29.92} points over Aegis-LlamaGuard and \textbf{21.62} over \texttt{gpt-4o}, respectively. Lastly, our guardrail synthetic data generation process that uses custom task-specific guardrail poli

==> sections/misc/data_descriptions.tex <==
\paragraph{Safety-Focused Datasets}
Here we describe safety-based training datasets used in our experiments. 
\newline
\textbf{BeaverTails}~\cite{ji2024beavertails}: This dataset provides over 300,000 question-answering pairs labeled with specific harm categories. It helps train models to identify and avoid generating harmful content.
\newline
\textbf{WildChat}~\cite{zhao2023inthe}: The BeaverTails dataset is a collection of question-answer pairs labeled for helpfulness and harmlessness, designed to train large language models (LLMs) to be safe and beneficial.  It includes over 300k QA pairs along with human ratings of their safety and usefulness, aiming to improve the alignment of LLMs with human values.
\newline
\textbf{BAD}~\cite{xu2021bot}: This dialogue dataset includes conversations where annotators attempt to elicit unsafe behaviors from a chatbot. All utterances are labeled as offensive or safe, aiding models in understanding safe communication.
\newline
\textbf{Real-Toxicity-Prompts}~\cite{gehman2020realtoxicityprompts}: This collection of 100,000 sentences is annotated with toxicity scores using the PERSPECTIVE API [30, 31]. It helps models learn to avoid generating toxic language.

\textbf{Helpfulness and Dialogue Datasets}
SHP [?]: This dataset consists of 385,000 human-labeled preferences regarding the helpfulness of responses to questions and instructions across various domains.
\newline
Anthropic-rr-rlhf [25, 18]: This collection includes human-annotated datasets on helpfulness and harmlessness, along with a red-teaming dataset containing prompts used as a foundation for our own experiments.


\paragraph{BeaverTails}
% https://huggingface.co/datasets/PKU-Alignment/BeaverTails
\paragraph{WildChat}

\paragraph{BAD [29] by MetaAI} A dialogue dataset in
which annotators attempt to elicit unsafe behaviors from the chat-bot using unsafe utterances, and
all utterances are annotated as offensive or safe.

\paragraph{REALTOXICITYPROMPTS} [16] consists of 100k
sentences annotated with toxicity scores from PERSPECTIVE API [30, 31]. 

\paragraph{SHP} A dataset consisting of 385k collective human preferences regarding the helpfulness of responses to questions and instructions across 18 different subject areas.

\paragraph{Anthropic-rr-rlhf} Anthropic contributed human-preference datasets about helpfulness and harmlessness [25] and a red teaming dataset [18] whose prompts serve as a basis for our dataset.


\paragraph{Safety-Focused Datasets}
Here we describe safety-based training datasets used in our experiments. 
\newline
\textbf{BeaverTails}~\cite{ji2024beavertails}: This dataset provides over 300,000 question-answering pairs labeled with specific harm categories. It helps train models to identify and avoid generating harmful content.
\newline
\textbf{WildChat}~\cite{zhao2023inthe}: The BeaverTails dataset is a collection of question-answer pairs labeled for helpfulness and harmlessness, designed to train large language models (LLMs) to be safe and beneficial.  It includes over 300k QA pairs along with human ratings of their safety and usefulness, aiming to improve the alignment of LLMs with human values.
\newline
\textbf{BAD}~\cite{xu2021bot}: This dialogue dataset includes conversations where annotators attempt to elicit unsafe behaviors from a chatbot. All utterances are labeled as offensive or safe, aiding models in understanding safe communication.
\newline
\textbf{Real-Toxicity-Prompts}~\cite{gehman2020realtoxicityprompts}: This collection of 100,000 sentences is annotated with toxicity scores using the PERSPECTIVE API [30, 31]. It helps models learn to avoid generating toxic language.

\textbf{Helpfulness and Dialogue Datasets}
SHP [?]: This dataset consists of 385,000 human-labeled preferences regarding the helpfulness of responses to questions and instructions across various domains.
\newline
Anthropic-rr-rlhf [25, 18]: This collection includes human-annotated datasets on helpfulness and harmlessness, along with a red-teaming dataset containing prompts used as a foundation for our own experiments.


\paragraph{BeaverTails}
% https://huggingface.co/datasets/PKU-Alignment/BeaverTails
\paragraph{WildChat}

\paragraph{BAD [29] by MetaAI} A dialogue dataset in
which annotators attempt to elicit unsafe behaviors from the chat-bot using unsafe utterances, and
all utterances are annotated as offensive or safe.

\paragraph{REALTOXICITYPROMPTS} [16] consists of 100k
sentences annotated with toxicity scores from PERSPECTIVE API [30, 31]. 

\paragraph{SHP} A dataset consisting of 385k collective human preferences regarding the helpfulness of responses to questions and instructions across 18 different subject areas.

\paragraph{Anthropic-rr-rlhf} Anthropic contributed human-preference datasets about helpfulness and harmlessness [25] and a red teaming dataset [18] whose prompts serve as a basis for our dataset.

==> sections/misc/llama_guard_finetuning.tex <==
\paragraph{Fine-tuning Llama-Base Architecture for Guardrail Response Generation}
We fine-tune the Llama-Base architecture to generate guardrail responses in the format "safe" or "unsafe: <rationale why it is unsafe>". The fine-tuning process is carried out using response-only loss, where the loss is minimized solely based on the generated response, without considering the prompt in the loss computation. The loss function for fine-tuning is defined as $L_{\text{resp}} = - \sum_i \log P(r_i | \theta)$ where $L_{\text{resp}}$ is the response-only loss, $r_i$ represents the tokens in the target response, and $\theta$ denotes the model parameters. Below we describe the two main aspects for improving the performance of our efficient safety guardrail LLMs: 1) generating synthetic data based on incorrect predictions from previous epochs and 2) alternating between response only supervised fine-tuning and prompt-tuning.

\subsection{Iterative Synthetic Data Generation and Retraining}
To improve the performance of our model, we employ a synthetic data generation process to create additional training data. This process is applied iteratively, where the model is fine-tuned on the augmented dataset after each round of data generation. After fine-tuning the model, we identify incorrect predictions and use them to generate synthetic training data. The incorrect predictions are retrieved using the following equation:

\begin{equation}
I = {(p_i, r_i) | \argmax_r P(r | p_i, \theta) \neq r_i}
\end{equation}

where $I$ is the set of incorrect predictions, $p_i$ is the input prompt, $r_i$ is the target response, and $\theta$ represents the fine-tuned model parameters.

The retrieved incorrect predictions are then used to generate synthetic training data using a data generation process similar to Evol-Instruct. The synthetic data is added to the existing training set, and the model is retrained using the updated dataset. This iterative process is carried out for a few iterations to progressively improve the model's performance.
The synthetic data generation algorithm consists of several key components. We generate compliant and non-compliant by first defining policy definitions to our synthetic data generation algorithm. The policy definition consists of the name of the policy (e.g "Avoid Unsafe Content"), a description (more detailed of what to guardrail against), a list of disallowed behaviors, a list of allowed behaviors and examples of both. The data generator (e.g Mixtral 8x22B-Instruct) then takes the policy definition, along with a set of parameteres that define the ratio of in-domain, borderline and jailbreaking prompts to generate non-compliant prompts. To increase linguistic diversity, a subset of the generated prompts undergo syntactic transformations, such as reversing the order of words or phrases, converting to lowercase or uppercase, repeating characters or substrings or modifying punctuation and whitespace.
We then generate a set of subtopics and writing styles based on the policy definition, followed by the generation of compliant prompts, non-compliants and borderline prompts that contain some ambiguity as to whether they are compliant or not.


\begin{itemize}
    \itemsep0em
    \item 
\end{itemize}

==> sections/misc/synthetic_data_gen.tex <==
\subsection{Iterative Synthetic Data Generation and Retraining}
To improve the performance of our model, we employ a synthetic data generation process to create additional training data. This process is applied iteratively, where the model is fine-tuned on the augmented dataset after each round of data generation. After fine-tuning the model, we identify incorrect predictions and use them to generate synthetic training data. The incorrect predictions are retrieved using the following equation:

\begin{equation}
I = {(p_i, r_i) | \argmax_r P(r | p_i, \theta) \neq r_i}
\end{equation}

where $I$ is the set of incorrect predictions, $p_i$ is the input prompt, $r_i$ is the target response, and $\theta$ represents the fine-tuned model parameters.

The retrieved incorrect predictions are then used to generate synthetic training data using a data generation process similar to Evol-Instruct. The synthetic data is added to the existing training set, and the model is retrained using the updated dataset. This iterative process is carried out for a few iterations to progressively improve the model's performance.


The synthetic data generation algorithm consists of several key components:

\subsubsection{Compliant Prompt Generation}
We generate compliant prompts that adhere to a given policy using multiple strategies:

\textbf{Diverse Prompts}: Generate diverse prompts based on seed prompts while ensuring policy compliance. The number of diverse prompts ($N_d$) is determined by
$N_d = round(r_d \times N_t)$ where $r_d$ is the diverse ratio and $N_t$ is the total number of prompts to generate.

\textbf{In-domain Prompts}: Generate in-domain prompts by conditioning on allowed behaviors and a set of subtopics related to the policy domain. The number of in-domain prompts ($N_i$) is calculated as $N_i = round(r_i \times N_t)$ where $r_i$ is the in-domain ratio.

\textbf{Inapplicable Prompts}: Generate prompts where the policy is not applicable. The number of inapplicable prompts ($N_p$) is determined by $N_p = round(r_p \times N_t)$
where $r_p$ is the inapplicable ratio.

\textbf{Jailbreak-inspired Prompts}: Generate compliant prompts inspired by jailbreak techniques to improve robustness. The number of jailbreak-inspired prompts ($N_j$) is calculated as $N_j = N_t - N_d - N_i - N_p$. The total number of compliant prompts generated is the sum of the above components as $N_c = N_d + N_i + N_p + N_j$. 


\subsubsection{Non-compliant Prompt Generation}
We generate non-compliant prompts that violate the policy using the following approaches:

\textbf{Diverse Prompts}: Similar to compliant prompt generation, diverse non-compliant prompts are created based on seed prompts.

\textbf{In-domain Prompts}: Generate in-domain non-compliant prompts by conditioning on disallowed behaviors and subtopics.

\textbf{Jailbreak-inspired Prompts}: Create non-compliant prompts using jailbreak techniques to improve the model's ability to identify policy violations. The total number of non-compliant prompts ($N_n$) is the sum of the above components.


\subsubsection{Prompt Augmentation}
To increase linguistic diversity, a subset of the generated prompts undergoes syntactic transformations, such as reversing the order of words or phrases, converting to lowercase or uppercase, repeating characters or substrings or modifying punctuation and whitespace. The probability of applying each transformation is controlled by a set of hyperparameters.

\subsubsection{Policy Refinement}
Based on the generated prompts and user feedback, the policy itself is iteratively refined to improve clarity and reduce contradictions. This involves 1) rewriting the policy for conciseness while preserving its meaning, 2) identifying and resolving contradictions or confusing aspects of the policy and 3) Updating the allowed and disallowed behaviors based on the generated prompts.

The synthetic data generation process is repeated for multiple iterations, with the model being fine-tuned on the augmented dataset after each iteration. This iterative approach allows for continuous improvement of the model's performance and robustness in understanding and adhering to the specified policy.

\subsection{Iterative Prompt-assisted Supervised Fine-tuning}
\paragraph{P-tuning for Guardrail Template Optimization}
After the iterative fine-tuning and synthetic data generation process, we employ p-tuning to further optimize the guardrail template text. P-tuning involves learning continuous prompt embeddings while keeping the already fine-tuned model parameters fixed. The objective of p-tuning is to minimize the following loss function: $L_{\text{p-tune}} = - \sum_i \log P(r_i | p_i, \theta_f, \theta_p)$ where $L_{p-tune}$ is the p-tuning loss, $p_i$ is the input prompt, $r_i$ is the target response, $\theta_f$ represents the fixed fine-tuned model parameters, and $\theta_p$ denotes the learnable prompt embeddings.

By optimizing the prompt embeddings through P-tuning, we aim to improve the model's ability to generate accurate and coherent guardrail responses while leveraging the knowledge acquired during the fine-tuning and iterative synthetic data generation process. The combination of fine-tuning, iterative synthetic data generation, and p-tuning allows us to create a robust and effective guardrail response generation system based on the Llama-Base architecture. This methodology enables the model to generate safe responses and provide informative rationales when the input is deemed unsafe, enhancing the overall quality and reliability of the generated responses.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{Styles/guardrail_llm_diagram.png}
    \caption{Guardrailing Process}
    \label{fig:guardrail_policy}
\end{figure}


\paragraph{Theory}
Let $\mathcal{D} = \{(x_i, y_i)\}_{i=1}^N$ be a dataset of prompt-response pairs, where $x_i$ is a prompt and $y_i$ is the corresponding response. First, we optimize the response-only loss. Let $f_\theta$ be a language model with parameters $\theta$. The response-only loss is: $\mathcal{L}_\text{resp}(\theta) = -\frac{1}{N}\sum_{i=1}^N \log p_\theta(y_i)$ where $p_\theta(y_i) = \prod_{t=1}^{|y_i|} p_\theta(y_{i,t} | y_{i,<t})$ is the probability of the response $y_i$ under the language model $f_\theta$. We optimize this loss to find the optimal parameters $\theta^*$ as $\theta^* = \arg\min_\theta \mathcal{L}_\text{resp}(\theta)$. Next, we fix the language model parameters to $\theta^*$ and optimize a prompt-tuning loss. Let $g_\phi$ be a prompt encoder with learnable parameters $\phi$ that maps a prompt $x_i$ to a continuous prompt embedding $z_i = g_\phi(x_i)$. The prompt-tuning loss is $\mathcal{L}_\text{prompt}(\phi) = -\frac{1}{N}\sum_{i=1}^N \log p_{\theta^*}(y_i | z_i)$ where $p_{\theta^*}(y_i | z_i) = \prod_{t=1}^{|y_i|} p_{\theta^*}(y_{i,t} | y_{i,<t}, z_i)$ is the probability of the response $y_i$ conditioned on the prompt embedding $z_i$ under the fixed language model $f_{\theta^*}$. We optimize this loss to find the optimal prompt encoder parameters $\phi^*$: $\phi^* = \arg\min_\phi \mathcal{L}_\text{prompt}(\phi)$.
Finally, we alternate between optimizing the response-only loss $\mathcal{L}_\text{resp}$ and the prompt-tuning loss $\mathcal{L}_\text{prompt}$ for a fixed number of iterations or until convergence: $\theta^{(k+1)} &= \arg\min_\theta \mathcal{L}_\text{resp}(\theta)$ and $\phi^{(k+1)} &= \arg\min_\phi \mathcal{L}_\text{prompt}(\phi; \theta^{(k+1)})$ where $k$ is the iteration number. The final model is defined by the parameters $(\theta^{(K)}, \phi^{(K)})$ after $K$ iterations.

